AC-VRNN: Attentive Conditional-VRNN for Multi-Future Trajectory Prediction

Anticipating human motion in crowded scenarios is essential for developing intelligent transportation systems, social-aware robots and advanced video surveillance applications. A key component of this task is represented by the inherently multi-modal nature of human paths which makes socially acceptable multiple futures when human interactions are involved. To this end, we propose a generative architecture for multi-future trajectory predictions based on Conditional Variational Recurrent Neural Networks (C-VRNNs). Conditioning mainly relies on prior belief maps, representing most likely moving directions and forcing the model to consider past observed dynamics in generating future positions. Human interactions are modeled with a graph-based attention mechanism enabling an online attentive hidden state refinement of the recurrent estimation. To corroborate our model, we perform extensive experiments on publicly-available datasets (e.g., ETH/UCY, Stanford Drone Dataset, STATS SportVU NBA, Intersection Drone Dataset and TrajNet++) and demonstrate its effectiveness in crowded scenes compared to several state-of-the-art methods.

==> packages.tex <==
\usepackage{graphicx}
\usepackage{amsmath,amssymb} % define this before the line numbering.
\usepackage{comment}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{xspace}
\usepackage[width=122mm,left=12mm,paperwidth=146mm,height=193mm,top=12mm,paperheight=217mm]{geometry}
\usepackage{soul}
\usepackage{enumitem}
\usepackage{caption}
\captionsetup[figure]{font=small,labelfont=small}
\captionsetup[table]{font=small,labelfont=small}
\usepackage{multirow}
\usepackage{algorithm}
\usepackage{algpseudocode}

\newcommand{\Linear}{\text{Linear}}
\newcommand{\MLP}{\text{MLP}}
\newcommand{\ReLU}{\text{ReLU}}
\newcommand{\Tanh}{\text{tanh}}
\newcommand{\Sigmoid}{\text{sigmoid}}
\newcommand{\Softplus}{\text{softplus}}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\KL}{KL}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\mathtext}[1]{\small{\textit{(#1)}}}
\newcommand{\Exp}[2]{\mathop{\mathbb{E}}_{#2}\left[#1\right]}
\newcommand{\vsigma}{\vec{\sigma}}
\newcommand{\pt}[2]{p(Z_{#1}|Z_{#2})}
\newcommand{\pth}{p_\theta}
\newcommand{\qph}{q_\phi} 
\newcommand{\Id}{\mathds{1}}
\newcommand{\dt}{\Delta}
\newcommand{\distt}[1]{\mathcal{N}(Z_{#1}+U_{#1}|\Delta \mathds{1})}
\newcommand{\cattwo}[2]{[#1\;\;#2]}
\newcommand{\catthr}[3]{[#1\;\;#2\;\;#3]}
\newcommand{\Prec}[1]{{\Sigma}_{#1}^{-1}}
\newcommand{\normtwo}[1]{\|#1\|_2}
\newcommand{\diff}{\textrm{\textit{diff}}}
\newcommand{\Normal}{\mathcal{N}}
\newcommand{\Ind}[1]{\mathbb{I}\left[#1\right]}
\newcommand{\lgsigsq}{\log\vec{\sigma}^2}
\newcommand{\deriv}[2]{\frac{\textit{\mathbf{d}}#1}{\textit{\mathbf{d}}#2}}
\newcommand{\vone}{\vec{\mathbf{1}}}
\newcommand{\vecx}{\vec{x}}
\newcommand{\vecu}{\vec{u}}
\newcommand{\vecz}{\vec{z}}
\newcommand{\bigCI}{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\meanfxn}{\textit{G}_{\alpha}}
\newcommand{\covfxn}{\textit{S}_{\beta}}
\newcommand{\emisfxn}{\textit{F}_{\kappa}}
\newcommand{\lthph}{\mathcal{L}(\vecx;(\theta, \phi))}
\newcommand{\qIndep}{\textbf{q-INDEP}}
\newcommand{\qLR}{\textbf{q-LR}}
\newcommand{\qRNN}{\textbf{q-RNN}}
\newcommand{\qBRNN}{\textbf{q-BRNN}}
\newcommand{\DKF}{DMM\xspace}
\newcommand{\DMM}{DMM\xspace}
\newcommand{\DKS}{\textbf{DKS}\xspace}

\newcommand{\bmx}[0]{\begin{bmatrix}}
\newcommand{\emx}[0]{\end{bmatrix}}
\newcommand{\qexp}[1]{\left<#1\right>}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\vects}[1]{\boldsymbol{#1}}
\newcommand{\matr}[1]{\mathbf{#1}}
\newcommand{\var}[0]{\operatorname{Var}}
\newcommand{\std}[0]{\operatorname{std}}
\newcommand{\cov}[0]{\operatorname{Cov}}
\newcommand{\matrs}[1]{\boldsymbol{#1}}
\newcommand{\va}[0]{\vect{a}}
\newcommand{\vb}[0]{\vect{b}}
\newcommand{\vc}[0]{\vect{c}}
\newcommand{\vh}[0]{\vect{h}}
\newcommand{\vv}[0]{\vect{v}}
\newcommand{\vx}[0]{\vect{x}}
\newcommand{\vz}[0]{\vect{z}}
\newcommand{\vw}[0]{\vect{w}}
\newcommand{\vf}[0]{\vect{f}}
\newcommand{\vi}[0]{\vect{i}}
\newcommand{\vo}[0]{\vect{o}}
\newcommand{\vy}[0]{\vect{y}}
\newcommand{\vg}[0]{\vect{g}}
\newcommand{\vm}[0]{\vect{m}}
\newcommand{\vu}[0]{\vect{u}}
\newcommand{\vL}[0]{\vect{L}}
\newcommand{\vr}[0]{\vect{r}}
\newcommand{\mW}[0]{\matr{W}}
\newcommand{\mG}[0]{\matr{G}}
\newcommand{\mX}[0]{\matr{X}}
\newcommand{\mQ}[0]{\matr{Q}}
\newcommand{\mU}[0]{\matr{U}}
\newcommand{\mV}[0]{\matr{V}}
\newcommand{\mA}{\matr{A}}
\newcommand{\mD}{\matr{D}}
\newcommand{\mS}{\matr{S}}
\newcommand{\mI}{\matr{I}}
\newcommand{\td}[0]{\text{d}}
\newcommand{\TT}[0]{\vects{\theta}}
\newcommand{\vepsilon}[0]{\vects{\epsilon}}
\newcommand{\valpha}[0]{\vects{\alpha}}
\newcommand{\vmu}[0]{\vects{\mu}}
\newcommand{\vzero}[0]{\vect{0}}
\newcommand{\tf}[0]{\text{m}}
\newcommand{\tdf}[0]{\text{dm}}
\newcommand{\grad}[0]{\nabla}
\newcommand{\alert}[1]{\textcolor{red}{#1}}
\newcommand{\N}[0]{\mathcal{N}}
\newcommand{\LL}[0]{\mathcal{L}}
\newcommand{\MM}[0]{\mathcal{M}}
\newcommand{\NN}[0]{\mathcal{N}}
\newcommand{\HH}[0]{\mathcal{H}}
\newcommand{\RR}[0]{\mathbb{R}}
\newcommand{\II}[0]{\mathbb{I}}
\newcommand{\Scal}[0]{\mathcal{S}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\E}[0]{\mathbb{E}}
\newcommand{\enabla}[0]{\ensuremath{%
    \overset{\raisebox{-0.3ex}[0.5ex][0ex]{%
    \ensuremath{\scriptscriptstyle e}}}{\nabla}}}
\newcommand{\enhnabla}[0]{\nabla_{\hspace{-0.5mm}e}\,}
\newcommand{\tred}[1]{\textcolor{red}{#1}}
\newcommand{\todo}[1]{{\Large\textcolor{red}{#1}}}
\newcommand{\done}[1]{{\Large\textcolor{green}{#1}}}
\newcommand{\dd}[1]{\ensuremath{\mbox{d}#1}}

\DeclareMathOperator*{\argmax}{\arg \max}
\DeclareMathOperator*{\argmin}{\arg \min}
\newcommand{\newln}{\\&\quad\quad{}}
\newcolumntype{?}{!{\vrule width 0.8pt}}

\newcommand{\Ax}{\mathcal{A}_x}
\newcommand{\Ay}{\mathcal{A}_y}
\newcommand{\ola}{\overleftarrow}
\newcommand{\ora}{\overrightarrow}
\newcommand{\ov}{\overline}
\newcommand{\tsr}{\rule{0pt}{2.6ex}}       % Top strut
\newcommand{\ms}{\rule{0pt}{0ex}}         % Middle strut
\newcommand{\bs}{\rule[-1.2ex]{0pt}{0pt}} % Bottom d strut
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
\newcommand{\pasquale}[1]{\textcolor{red}{#1}}
\newcommand{\alessia}[1]{\textcolor{blue}{#1}}
\newcommand{\lamberto}[1]{\textcolor{green}{#1}}
